REvolveR: Continuous Evolutionary Models for Robot-to-robot Policy Transfer

A popular paradigm in robotic learning is to train a policy from scratch for every new robot. This is not only inefficient but also often impractical for complex robots. In this work, we consider the problem of transferring a policy across two different robots with significantly different parameters such as kinematics and morphology. Existing approaches that train a new policy by matching the action or state transition distribution, including imitation learning methods, fail due to optimal action and/or state distribution being mismatched in different robots. In this paper, we propose a novel method named $REvolveR$ of using continuous evolutionary models for robotic policy transfer implemented in a physics simulator. We interpolate between the source robot and the target robot by finding a continuous evolutionary change of robot parameters. An expert policy on the source robot is transferred through training on a sequence of intermediate robots that gradually evolve into the target robot. Experiments on a physics simulator show that the proposed continuous evolutionary model can effectively transfer the policy across robots and achieve superior sample efficiency on new robots. The proposed method is especially advantageous in sparse reward settings where exploration can be significantly reduced. Code is released at https://github.com/xingyul/revolver.

==> figure_dapg_v1.tex <==
\begin{figure}[ht]
\centering
\newcommand\dapgwidth{0.16}
\subfloat[\texttt{Hammer} environment. ]{
\begin{tabular}{c}
\addvbuffer[0pt 0pt]{\includegraphics[width=\dapgwidth\textwidth, valign=m]{Figures/dapg/hammer_0.jpg}} $\rightarrow$ \addvbuffer[0pt 0pt]{\includegraphics[width=\dapgwidth\textwidth,valign=m]{Figures/dapg/hammer_1.jpg}}
\end{tabular} 
} 
\vspace{-2ex}
\\
\subfloat[\texttt{Relocate} environment. ]{
\begin{tabular}{c}
\addvbuffer[0pt 0pt]{\includegraphics[width=\dapgwidth\textwidth, valign=m]{Figures/dapg/relocate_0.jpg}} $\rightarrow$ \addvbuffer[3pt 0pt]{\includegraphics[width=\dapgwidth\textwidth,valign=m]{Figures/dapg/relocate_1.jpg}} 
\end{tabular} 
} 
\vspace{-2ex}
\\
\subfloat[\texttt{Door} environment. ]{
\begin{tabular}{c}
\addvbuffer[0pt 0pt]{\includegraphics[width=\dapgwidth\textwidth, valign=m]{Figures/dapg/door_0.jpg}} $\rightarrow$ \addvbuffer[3pt 0pt]{\includegraphics[width=\dapgwidth\textwidth,valign=m]{Figures/dapg/door_1.jpg}} \\
\end{tabular}
} 
\vspace{-1ex}
\caption{\textbf{Hand Manipulation Suite tasks.}
(a) \texttt{Hammer} environment. The goal is to pick up the hammer and smash the nail into the board;
(b) \texttt{Relocate} environment. The goal is to pick up the blue ball and take it to the desired site denoted as green sphere;
(c) \texttt{Door} environment. The goal is to switch the latch and fully open the door.
}
\label{fig:dapg}
\end{figure}



==> figure_gym.tex <==
\begin{figure}[t]
\centering
\newcommand\antwidth{0.12}
\newcommand\humanoidwidth{0.16}
\subfloat[\texttt{Ant-length-mass}]{
\begin{tabular}{c}
\addvbuffer[0pt 0pt]{\includegraphics[width=\antwidth\textwidth, valign=m]{Figures/gym/ant_leg_length_mass_interp_0.00.jpg}} $\rightarrow$ \addvbuffer[0pt 0pt]{\includegraphics[width=\antwidth\textwidth,valign=m]{Figures/gym/ant_leg_length_mass_interp_1.00.jpg}}
\end{tabular} 
} 
\\
\vspace{-3ex}
\subfloat[\texttt{Humanoid-length-mass}]{
\begin{tabular}{c}
\addvbuffer[0pt 0pt]{\includegraphics[height=\humanoidwidth\textwidth, valign=m]{Figures/gym/huamoid_leg_length_mass_interp_0.00.jpg}} $\rightarrow$ \addvbuffer[3pt 0pt]{\includegraphics[height=\humanoidwidth\textwidth,valign=m]{Figures/gym/huamoid_leg_length_mass_interp_1.00.jpg}} 
\end{tabular} 
} 
\\
\vspace{-2ex}
\subfloat[\texttt{Ant-leg-emerge}]{
\begin{tabular}{c}
\addvbuffer[0pt 0pt]{\includegraphics[width=\antwidth\textwidth, valign=m]{Figures/gym/ant_leg_emerge_interp_0.00.jpg}} $\rightarrow$ \addvbuffer[3pt 0pt]{\includegraphics[width=\antwidth\textwidth,valign=m]{Figures/gym/ant_leg_emerge_interp_1.00.jpg}} \\
\end{tabular}
} 
\caption{Source-to-target robot evolution in the MuJoCo Gym environment used in experiments.
}
\end{figure}



==> unused.tex <==

Note that when $h\rightarrow\infty$, the optimization objective in Equation \eqref{eq:local:reward:opt} is reduce to
\begin{equation} \label{eq:local:reward:opt:infty}
\begin{split}
    \max_{\pi}
    \mathop{\mathbb{E}}_{ 
    \substack{
    a_t \sim \pi(\cdot \mid s_t) \\ 
    s_{t+1} \sim M(\cdot \mid s_t, a_t)
    }}
    [\sum_{t} \gamma^t r_t]
\end{split}
\end{equation}
where $M = E(\alpha_k + \delta)$,
which is essentially deterministic in Equation \eqref{eq:det:opt} with evolution progression size $l_{k+1}$ equals to the neighborhood range $\delta$.


\begin{equation}
\begin{split}
    f(\alpha^\prime) & = (1+h\alpha^\prime)V^{\pi^*_{E(\alpha^\prime)},E(\alpha^\prime)}- \frac{1}{\delta} \int_{\beta=\alpha}^{\alpha+\delta} (1 + h \beta)
    V^{\pi^*_{E(\alpha^\prime)},E(\beta)}  \dd{\beta} \\
    & = \int_{\beta=\alpha}^{\alpha+\delta} (V^{\pi^*_{E(\alpha^\prime)},E(\alpha^\prime)} - V^{\pi^*_{E(\alpha^\prime)},E(\beta)} ) + h 
\end{split}
\end{equation}
is maximized at $\alpha^\prime$
\begin{equation}
\begin{split}
    & \lim_{\delta \rightarrow 0}
    \left[
    \mathop{\arg\max}_{\pi}
    \mathop{\mathbb{E}}_{ 
    \substack{
    \beta \sim U([\alpha, \alpha+\delta])
    }}
    \mathop{\mathbb{E}}_{ 
    \substack{(s_t, a_t) \sim \pi, E(\beta)
    }}
    \sum_{t} \gamma^t r_t (1 + h \beta)
    \right] \\
    & = \lim_{\delta \rightarrow 0}
    \left[
    \mathop{\arg\max}_{\pi}
    \mathop{\mathbb{E}}_{ 
    \substack{
    \beta \sim U([\alpha, \alpha+\delta])
    }}
    (1 + h \beta)
    \mathop{\mathbb{E}}_{ 
    \substack{(s_t, a_t) \sim \pi, E(\beta)
    }}
    \sum_{t} \gamma^t r_t 
    \right] \\
    & = \lim_{\delta \rightarrow 0}
    \left[
    \mathop{\arg\max}_{\pi}
    \mathop{\mathbb{E}}_{ 
    \substack{
    \beta \sim U([\alpha, \alpha+\delta])
    }}
    (1 + h \beta) V^{\pi, E(\beta)} 
    \right] \\
    & = \lim_{\delta \rightarrow 0}
    \left[
    \mathop{\arg\max}_{\pi}
    \int_{\beta=\alpha}^{\alpha+\delta} (1+h\beta)
    \right] \\
\end{split}
\end{equation}
    
    
    
    By the assumption in Equation \ref{eq:alpha:lipschitz:assumption},
\begin{equation}
\begin{split}
  \exists \delta > 0, \text{s.t. } \forall |\alpha^\prime - \alpha | < \delta, 
 ||E(\alpha)(s) - E(\alpha^\prime)(s)|| \le L_1 |\alpha - \alpha^\prime|,
 \forall s\in\mathcal{S} 
\end{split}
\end{equation}
